Loss Landscape Dependent Self-Adjusting Learning Rates in Decentralized Stochastic Gradient Descent

Distributed Deep Learning (DDL) is essential for large-scale Deep Learning (DL) training. Synchronous Stochastic Gradient Descent (SSGD) 1 is the de facto DDL optimization method. Using a sufficiently large batch size is critical to achieving DDL runtime speedup. In a large batch setting, the learning rate must be increased to compensate for the reduced number of parameter updates. However, a large learning rate may harm convergence in SSGD and training could easily diverge. Recently, Decentralized Parallel SGD (DPSGD) has been proposed to improve distributed training speed. In this paper, we find that DPSGD not only has a system-wise run-time benefit but also a significant convergence benefit over SSGD in the large batch setting. Based on a detailed analysis of the DPSGD learning dynamics, we find that DPSGD introduces additional landscape-dependent noise that automatically adjusts the effective learning rate to improve convergence. In addition, we theoretically show that this noise smoothes the loss landscape, hence allowing a larger learning rate. We conduct extensive studies over 18 state-of-the-art DL models/tasks and demonstrate that DPSGD often converges in cases where SSGD diverges for large learning rates in the large batch setting. Our findings are consistent across two different application domains: Computer Vision (CIFAR10 and ImageNet-1K) and Automatic Speech Recognition (SWB300 and SWB2000), and two different types of neural network models: Convolutional Neural Networks and Long Short-Term Memory Recurrent Neural Networks.

==> Makefile <==
.SUFFIXES: .eps .pdf
LATEX=./colourlatex.sh pdflatex
BIBTEX=bibtex
FIG2DEV=fig2dev

MAIN=main
#SUP=supplementary
#BIBMAIN=acmsmall-sample-bibfile
BIBMAIN=refs

all: $(MAIN).pdf #$(SUP).pdf #$(MAIN).ps

#FIGSEPS=$(shell ls -1 figs/*.eps)

#RESULTSEPS=$(shell ls -1 results/*.eps)

#EPS=$(FIGSEPS) $(RESULTSEPS)




MAINTEX=$(MAIN).tex \
    $(BIBMAIN).bib \

$(MAIN).pdf: $(MAINTEX) $(EPS) $(BIBMAIN).bbl
	@echo Compiling $(MAIN)
	@$(LATEX) $(MAIN)
	@$(MAKE) fixlabels

# SUPTEX=$(SUP).tex \
#     $(BIBMAIN).bib \

# $(SUP).pdf: $(SUPTEX) $(EPS) $(BIBMAIN).bbl
# 	@echo Compiling $(SUP)
# 	@$(LATEX) $(SUP)
# 	@$(MAKE) fixlabels
 

# $(MAIN).pdf: $(MAIN).dvi
# 	@dvipdfmx -p letter $(MAIN).dvi

# $(MAIN).ps: $(MAIN).dvi
# 	@dvips $(MAIN).dvi
# 	@pkill -HUP -f "^gv .*$@" || true


fixlabels:
ifneq ($(shell grep -s -c 'Label(s) may have changed. Rerun to get cross-references right.' $(MAIN).log),0)
	@echo $(MAIN) Compiling again to fix labels
	@$(LATEX) $(MAIN)
else
	@echo $(MAIN) Labels are correct
endif

$(BIBMAIN).bbl: $(BIBMAIN).bib 
	@echo Compiling required EPS files
	#@make -C figs
	@echo Compiling main for bibliography
	@$(LATEX) $(MAIN)
	@echo Generating bibliography
	@$(BIBTEX) $(MAIN)
	@echo Recompiling main after generating bibliography
	@$(LATEX)  $(MAIN)
	@$(MAKE) fixlabels
	# @echo Compiling SUP for bibliography
	# @$(LATEX) $(SUP)
	# @echo Generating bibliography
	# @$(BIBTEX) $(SUP)
	# @echo Recompiling SUP after generating bibliography
	# @$(LATEX)  $(SUP)
	# @$(MAKE) fixlabels

%.eps.pdf: %.eps
	@echo "	" Converting $< to $(@)
	@epstopdf --outfile=figs/$(@) $<

clean:
	#@make -C figs clean
	@/bin/rm -f $(MAIN).ps $(MAIN).pdf *.aux *.dvi *.log *.bbl *.blg figs/*.pdf figures/plot/*.pdf *.toc *.out *.bak *.*~


==> checklist.tex <==
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}

% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

 \begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Not code(proprietary), but enough instructions to reproduce the results. }
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> data/cifar10/2dcontour/README <==
      model
     /    \
    SYNC  DPSGD
  / \        / \
 e1 e20     e1 e20



==> data/cifar10/2dcontour/README_ <==
      model
     /    \
    SYNC  DPSGD
  / \        / \
 e1 e20     e1 e20

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> rebuttal/experiments.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
%\vspace{-0.13in}
\begin{tiny}
\begin{table}[b]
\footnotesize
\vspace{-0.25in}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\hline
                                                                    &            & Eff-b0 & SE-18 & Res-18 & Dense-121 & Mobile & Google & ResNext-29 & SWB-2000 \\ \hline
                                                                    & Single-GPU & 2.92   & 1.58  & 1.37   & 5.48      & 1.02   & 5.31   & 4.55       & 203.21   \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Latency\\ (1$\mu$s)\end{tabular}} & SSGD       & 0.34   & 0.39  & 0.35   & 0.68      & 0.17   & 0.58   & 0.56       & 38.00    \\ \cline{2-10} 
                                                                    & DPSGD      & 0.26   & 0.31  & 0.32   & 0.58      & 0.12   & 0.49   & 0.41       & 29.71    \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Latency\\ (1$m$s)\end{tabular}} & SSGD       & 0.46   & 0.85  & 0.82   & 0.96      & 0.30   & 0.84   & 0.94       & 96.31   \\ \cline{2-10} 
                                                                    & DPSGD      & 0.27   & 0.31  & 0.32   & 0.58      & 0.13   & 0.50   & 0.42       & 29.85    \\ \hline
\end{tabular}
\caption{Time (hours) to complete training  with batch size 128 per GPU and 16 GPUs in total.}
\vspace{-0.3in}
\end{table}
\end{tiny}
%\vspace{-0.2in}
%
%
% Distributed deep learning is a multi-objective process, which aims at optimizing both runtime and convergence . Batch size is key to the parallelism exploitable and thus dictates the runtime performance. When using the same batch size running the same number epochs (i.e., the same level of parallelism and same computation workload), the runtime benefits of DPSGD is  well-established in the literature (cite dpsgd, adpsgd, adpsgd-fb) and we summarize them here: (1) The total size of messages transferred from each learner in DPSGD is half of that in SSGD (2) Orders of magnitude of fewer number of handshake messages in DPSGD than in SSGD (3) DPSGD enables asynchronous computing to avoid the straggler problem. Table 1 list the runtime performance under batch size 2048 for CIFAR10 experiment, and we can clearly see that DPSGD runs faster than SSSGD. Due to space limit, we omit all the other setup numbers as they exhibit the same trend. In essence, the theoretical linear speedup of DPSGD is proven in cite[dpsgd] while enjoying the faster communication performance mentioned agove. In another word, when the batch size is the same, DPSGD runs inherently faster than SSGD. The focus of this paper is to establish that DPSGD also converges better under the same batch size (especially when the batch size is large). Together, we demonstrate DPSGD dominates SSGD in both runtime and convergence performance.
%
%\vspace*{-0.05in}
{\bf Experiments} \textit{(1) Number of epochs.} In all DPSGD and SSGD experiments we used the \textit{same} number of epochs as in the well-tuned single-GPU baseline. We included convergence w.r.t epochs plots in Appendix-B. \textit{(2) Learning rate tuning.} We explored different learning rates for DPSGD and SSGD in the large batch setting (Tables 5$\&$6 in paper). Bold text in each column indicates the best accuracy achieved for that model \textit{across} different learning rate and optimization method configurations. DPSGD consistently achieves highest accuracy, all learning rates considered. \textit{(3) Wall-clock time.} DPSGD inherently runs faster than SSGD (i.e., less messages transmitted, tolerance of high-latency network)[13]. Table 1 below records training time for each representative task (batch size 128 per GPU, 16 GPUs) for both low and high latency networks. Other tasks and batch-size setups show the same trend: DPSGD runs faster than SSGD.  \textit{(4) Time to reach target accuracy.} DPSGD runs faster than SSGD when running with the same batch-size. Note for Eff-B0 (target accuracy 90\%) and SWB-2000 (target heldout loss 1.48), DPSGD reaches target accuracy with twice the batch size as used in SSGD, all learning rates considered (Tables 5 $\&$6). Thus DPSGD can effectively use 2X more GPUs. DPSGD achieves target accuracy for Eff-B0 in 0.067 hours and for SWB-2000 in 10.08 hours (64 GPUs). In contrast, SSGD achieves target accuracy for Eff-B0 in 0.19 hours and for SWB-2000 in 23.15 hours (32 GPUs).
\textit{(5) DPSGD with many learners.} Each learner \textit{randomly} picks \textit{one} neighbor to communicate in each iteration, which improves large-scale DPSGD training efficiency [15]. \textit{(6) Large-scale experiment.} SWB-2000 is more challenging than ImageNet. It takes over 200 hours on 1 V100 GPU to finish training SWB-2000. SWB-2000 has 32,000 highly unevenly distributed classes whereas ImageNet has 1000 evenly distributed classes. \textit{(7) Figure 3.} Setup of Figure 3 is described from line 197 to line 203, which follows [29].  DPSGD has smoother landscape (colder color) than SSGD.

==> rebuttal/experiments_backup.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
%\vspace{-0.13in}
\begin{tiny}
\begin{table}[htp]
\footnotesize
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\hline
                                                                    &            & Eff-b0 & SE-18 & Res-18 & Dense-121 & Mobile & Google & ResNext-29 & SWB-2000 \\ \hline
                                                                    & Single-GPU & 2.92   & 1.58  & 1.37   & 5.48      & 1.02   & 5.31   & 4.55       & 203.21   \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Latency\\ (1$\mu$s)\end{tabular}} & SSGD       & 0.34   & 0.39  & 0.35   & 0.68      & 0.17   & 0.58   & 0.56       & 38.00    \\ \cline{2-10} 
                                                                    & DPSGD      & 0.26   & 0.31  & 0.32   & 0.58      & 0.12   & 0.49   & 0.41       & 29.71    \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Latency\\ (1$m$s)\end{tabular}} & SSGD       & 0.46   & 0.85  & 0.82   & 0.96      & 0.30   & 0.84   & 0.94       & 96.31   \\ \cline{2-10} 
                                                                    & DPSGD      & 0.27   & 0.31  & 0.32   & 0.58      & 0.13   & 0.50   & 0.42       & 29.85    \\ \hline
\end{tabular}
\caption{Time (hours) to complete training  with batch size 128 per GPU and 16 GPUs in total.}
\end{table}
\end{tiny}
\vspace{-0.2in}
%
%
% Distributed deep learning is a multi-objective process, which aims at optimizing both runtime and convergence . Batch size is key to the parallelism exploitable and thus dictates the runtime performance. When using the same batch size running the same number epochs (i.e., the same level of parallelism and same computation workload), the runtime benefits of DPSGD is  well-established in the literature (cite dpsgd, adpsgd, adpsgd-fb) and we summarize them here: (1) The total size of messages transferred from each learner in DPSGD is half of that in SSGD (2) Orders of magnitude of fewer number of handshake messages in DPSGD than in SSGD (3) DPSGD enables asynchronous computing to avoid the straggler problem. Table 1 list the runtime performance under batch size 2048 for CIFAR10 experiment, and we can clearly see that DPSGD runs faster than SSSGD. Due to space limit, we omit all the other setup numbers as they exhibit the same trend. In essence, the theoretical linear speedup of DPSGD is proven in cite[dpsgd] while enjoying the faster communication performance mentioned agove. In another word, when the batch size is the same, DPSGD runs inherently faster than SSGD. The focus of this paper is to establish that DPSGD also converges better under the same batch size (especially when the batch size is large). Together, we demonstrate DPSGD dominates SSGD in both runtime and convergence performance.
%
{\bf Experiments} \textit{(1) Number of epochs:} In all DPSGD and SSGD experiments we used the \textit{same} number of epochs as in the well-tuned single-GPU baseline. We included convergence w.r.t epochs plots in Appendix-B. \textit{(2) Learning rate tuning} We explored different learning rates for DPSGD and SSGD in the large batch setting (Tables 5$\&$6 in paper). Bold text in each column indicates the best accuracy achieved for that model \textit{across} different learning rate and optimization method configurations. DPSGD consistently achieves highest accuracy, all learning rates considered. \textit{(3) Wall-clock time} DPSGD's inherent runs faster than SSGD (i.e., less messages transmitted, tolerance of high-latency network)[13]. Table 1 above records training time for each representative task (batch size 128 per GPU, 16 GPUs) for both low and high latency networks. Other tasks and batch-size setups show the same trend: DPSGD runs faster than SSGD.  \textit{(4) Time to reach target accuracy} DPSGD runs faster than SSGD when running with the same batch-size. Note for Eff-B0 (target accuracy 90\%) and SWB-2000 (target heldout loss 1.48), DPSGD reaches target accuracy with twice the batch size as used in SSGD, all learning rates considered (Table 5 $\&$6). Thus DPSGD can effectively use 2X more GPUs. DPSGD achieves target accuracy for Eff-B0 in 0.067 hours and for SWB-2000 in 10.08 hours (64 GPUs). In contrast, SSGD achieves target accuracy for Eff-B0 in 0.19 hours and for SWB-2000 in 23.15 hours (32 GPUs).
\textit{(5) DPSGD with many learners} Each learner \textit{randomly} picks \textit{one} neighbor to communicate in each iteration, which improves large-scale DPSGD training efficiency [15]. \textit{(6) Large-scale experiment} SWB-2000 is more challenging than ImageNet. It takes over 200 hours on 1 V100 GPU to finish training SWB-2000. SWB-2000 has 32,000 highly unevenly distributed classes whereas ImageNet has 1000 evenly distributed classes. \textit{(7) Figure 3} Setup of Figure 3 is described from line 197 to line 203, which follows [29].  DPSGD has smoother landscape (colder color) than SSGD.

==> rebuttal/theory_yuhai.tex <==
{\bf Theory parts.} %The reviewers' questions fall into two categories. 
{\it (1) The self-adjusted  effective learning rate $\alpha_e$ in DPSGD.} %As shown in our paper, $\alpha_e$ decreases as the noise strength ($\Delta$) increases. 
We agree with reviewer 1 that due to the different learning paths in different algorithms $\alpha_e$ in DPSGD is not always smaller than that in SSGD at all times, which is clearly shown in Fig. 1A in our paper. However, this is not the point
%\vspace*{-0.12in}
\begin{wrapfigure}{l}{0.25\textwidth}
%\captionsetup{labelformat=nonumber}
\begin{tiny}
\vspace*{-0.2in}
\centering
     \includegraphics[width=0.25\textwidth]{./Delta_v2.eps}
     \label{fig:eff-noise}
\vspace*{-0.2in}
\caption{\small{The additional DPSGD noise $\Delta^{(2)}\gg \Delta_{S}$ in the beginning of the training before it decreases to become comparable to $\Delta_{S}$. }}
%The additional DPSGD noise $\Delta^{(2)}\gg \Delta_{S}$ in the beginning of the training before it decreases to become comparable to $\Delta_{S}$
    \label{fig:noise}
    \vspace*{-0.3in}
    \hspace*{-0in}
\end{tiny}
\end{wrapfigure}
%\vspace*{-0.005in}
%the point 
we try to make. Our key result here is that $\alpha_e$ in DPSGD is self-adjusted via its dependence on the noise.
As shown in Fig.~1A (lower panel) in our paper, $\alpha_e$ in DPSGD is reduced significantly in the beginning of the training process which helps avoid overshoot for a large learning rate $\alpha (=1)$; afterwards it recovers to $\approx \alpha$ so that a fast training time is maintained (this answers one of reviewer 2's questions).
The reason for this self-adjusted $\alpha_e$ in DPSGD is that the DPSGD noise $\Delta_{DP}$ can be decomposed into the SSGD noise $\Delta_S$ evaluated at the mean weight $\vec{w}_a$ plus an additional noise $\Delta^{(2)}(>0)$ that originates from the difference in local weights ($\vec{w}_j$) for individual learners from their mean ($\vec{w}_a$): $\Delta_{DP}=\Delta_{S}+\Delta^{(2)}$. 
By expanding $\Delta^{(2)}$ w.r.t. $\Delta \vec{w}_j \equiv \vec{w}_j-\vec{w}_a$, we obtain the average $\Delta^{(2)}$ over minibatch ensemble $\{\mu\}$:
\vspace*{-0.04in}

%$\Delta \dec{w}_j=depends on the loss function landscape, in particular,     %The noise in all SGD-based algorithms (including SSGD and DPSGD studied in this paper) is due to the difference between the minibatch gradient and the whole batch gradient at a given weight vector. Therefore, the noise strength is not a constant and it varies in the weight space. The effective learning rate $\alpha_e$ defined in our paper also varies in the weight space and the equation in L95 mentioned by the reviewer relates the noise strength and the effective learning rate at a given weight vector w. As shown Eq~8 in Appendix A, at a given weight vector w, the DPSGD noise strength is larger than the SSGD noise by an additional non-negative term $\Delta^{(2)}$ that originates from the difference in local weights for individual learners in DPSGD. Thus, the equation in L95 indicates that the effective learning rate in DPSGD is smaller than that of SSGD at the same weight point in the weight-space. 
%As pointed out by reviewer #1, 
%since different algorithms (DPSGD and SSGD) lead to different learning path, the equation in L95 does not prove that the DPSGD algorithm always has a smaller effective learning rate than SSGD for any given time (or iteration). But this is not the point we try to make in this paper. Indeed, as shown in Fig. 1A (lower panel) in our paper, the DPSGD learning rate (green line) becomes comparable (bigger and smaller) as the SSGD (red line) in the latter stage of the learning process ($t>700$). However, during the initial learning stage ($0<t<700$), the DPSGD learning rate is significantly reduced as clearly shown in Fig. 1A. It is this reduction in $\alpha_e$ in the beginning of the learning process when the landscape is rough that prevents the overshoot of the algorithm when the original learning rate $\alpha$ is large. Once the algorithm starts to converge, i.e., when the loss landscape becomes smoother, the $\alpha_e$ in DPSGD recovers to be approximately $\alpha$. This landscape-dependent learning rate in DPSGD is one of the main findings in our paper.  The reason for this self-adjusted reduction of the effective learning rate in DPSGD can be understood by looking at the dominant DPSGD noise $\Delta^{(2)}$ given in Appendix A:
%\vspace*{-0.05in}
\begin{small}
\begin{equation}
   %\vspace*{-0.03in}
  \langle \Delta^{(2)}\rangle_\mu \equiv \langle ||n^{-1}\sum_{j=1}^n[\nabla L^{\mu_j}(\vec{w}_j)- \nabla L^{\mu_j}(\vec{w}_a)]||^2\rangle_\mu
    \approx \sum_{k,l,l'} H _{kl}H_{kl'} C_{ll'},
    %\approx \sum_{k,l,l'} \nabla^2 _{kl}L^{\mu_j}\nabla^2 _{kl'}L^{\mu_j} C_{ll'} %=tr(H C H^{T})
    %  \vspace*{-0.01in}
    \label{D2}
\end{equation}
\end{small}
%\vspace*{-0.03in}
where $H_{kl}=\nabla^2 _{kl}L$ is the Hessian matrix of the loss function and $C_{ll'}=n^{-2}\sum_{j=1}^n \Delta w_{j,l} \Delta w_{j,l'}$ is the weight covariance matrix. Eq.~\ref{D2} shows that $\Delta^{(2)}$ is large in the beginning of the training process when the loss landscape is rough with large curvatures, which leads to a reduced $\alpha_e$; $\Delta^{(2)}$ decreases as the system reaches the smooth part of the landscape where $\alpha_e$ recovers back to $\alpha$. This behavior of the additional DPSGD noise $\Delta^{(2)}$ is verified in our MNIST numerical experiments as shown in Figure 1 above. 
% \begin{wrapfigure}{l}{0.30\textwidth}
% %\small
% \vspace{-0.3in}
% \centering
%       \includegraphics[width=0.30\textwidth]{./Delta.pdf}
%       \label{fig:eff-noise}
% \vspace*{-0.3in}
% \caption{Noise effect.}
%     \label{fig:noise}
%     \vspace*{-0.45in}
%     \hspace*{-0.3in}
% \end{wrapfigure}
%
%
%
%This landscape dependence of $\Delta^{(2)}$ explains the self-adjusted $\alpha_e$ behavior in DPSGD shown in Fig. 1A in our paper. %Specifically, $\alpha_e$ in DPSGD is reduced significantly in the beginning of the training process which help avoid the overshoot problem; afterwards it recovers to the large initial learning rate $\alpha$ so that a fast training time is maintained. %as $\alpha_e$ . %leads to an effective learning rate that is much reduced in the beg  Quantitatively, for the MNIST experiments, we have computed $\Delta^{(2}}$ which shows that it is much larger than the SSGD noise $\Delta^{(1)}$ along the same trajectory
%
% \begin{figure*}[t]%[!htpb]
% \small
% \centering
%       \includegraphics[width=0.33\columnwidth]{./Delta.pdf}
%       \label{fig:eff-noise}
% \caption{Noise effect.}
%     \label{fig:noise}
%     %\vspace*{-0.2in}
% \end{figure*}
%{\bf The effects of noise in different algorithms.}
{\it (2) How does DPSGD noise help find generalizable solutions.} It is known that directly adding noise with a constant strength to learning dynamics does not improve generalization [r1]. The reason is that a “successful noise” should depend on the loss landscape [17,r2] -- larger when the landscape is rougher to help escape from local traps; smaller when the landscape is smoother and flatter to find and stay at good solutions. %In order to improve generalization performance, the strength of the injected noise needs to be fine-tuned, e.g. by adding time-dependent annealing noise (Arvind,2016) or adding curvature dependent noise (Zhu,2019). % Thus a “successful noise” should be large enough to allow efficient search to find a solution in the high dimensional weight-space, and also needs to be small enough to allow the network to converge to a solution. Furthermore, even if algorithms with an injected noise could be tuned to allow them to find solutions, they would not actively seek the flat minima solutions which have lower generalization error because the injected noise has a constant strength independent of the landscape shape (such as its curvature or flatness).
Since noise in SGD-based algorithms is caused by the difference between minibatch gradients and the whole batch gradient, it naturally depends on the loss function landscape. In particular, the SGD noise strength is found to be inversely dependent on the flatness of the loss function [18] %(Feng and Tu, 2019)
, which helps the system find flat minima where the solutions have been argued to be more generalizable [8,23]. However, besides its landscape dependence, SGD noise also depends inversely on the minibatch size $B$ [17]. With $n$ synchronized learners, the noise in SSGD scales as $1/(nB)$, which is too small to be effective for a large batch size $nB$. A main finding of our paper is that the additional landscape-dependent noise $\Delta^{(2)}$ in DPSGD can make up for the small SSGD noise when $nB$ is large and help find flat minima with good generalization performance.\\
\vspace*{-0.01in}
[r1] An. The effects of adding noise during backpropagation training on a generalization performance. 1996.\\
\vspace*{-0.05in}
[r2] Zhu et al. The Anisotropic Noise in Stochastic Gradient Descent. ICML 2019. 
%Its Behavior of Escaping from Sharp Minima and Regularization Effects. ICML 2019.
% \vspace*{-0.05in}
% \begin{itemize}
% \begin{small}
% \item [r1] An 1996. The effects of adding noise during backpropagation training on a generalization performance.
% \item [r2] Zhu et al. 2019. The Anisotropic Noise in Stochastic Gradient Descent: Its Behavior of Escaping from Sharp Minima and Regularization Effects.
% \end{small}
% \end{itemize}
% \vspace*{-0.05in}










